The stack calculus

We introduce a functional calculus with simple syntax and operational semantics in which the calculi introduced so far in the Curry-Howard correspondence for Classical Logic can be faithfully encoded. Our calculus enjoys confluence without any restriction. Its type system enforces strong normalization of expressions and it is a sound and complete system for full implicational Classical Logic. We give a very simple denotational semantics which allows easy calculations of the interpretation of expressions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{93}
\providecommand{\publicationstatus}{D. Kesner and P. Viana (Eds.): LSFA 2012\\
EPTCS 113, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.113.10}{10.4204/EPTCS.113.10}}

